Optimal Adaptive Learning in Uncontrolled Restless Bandit Problems

In this paper we consider the problem of learning the optimal policy for uncontrolled restless bandit problems. In an uncontrolled restless bandit problem, there is a finite set of arms, each of which when pulled yields a positive reward. There is a player who sequentially selects one of the arms at each time step. The goal of the player is to maximize its undiscounted reward over a time horizon T. The reward process of each arm is a finite state Markov chain, whose transition probabilities are unknown by the player. State transitions of each arm is independent of the selection of the player. We propose a learning algorithm with logarithmic regret uniformly over time with respect to the optimal finite horizon policy. Our results extend the optimal adaptive learning of MDPs to POMDPs.

==> chap_strong.tex <==
In this chapter we study the single-agent uncontrolled restless bandit problem. We propose an algorithm with logarithmic strong regret under Markovian transition probabilities for the arms. The organization of this chapter is as follows. Problem definition, notations and several assumptions are given in Section \ref{single:sec:strong-probform}. Restless bandit problem with single play is investigated, and an algorithm with logarithmic strong regret is proposed in Section \ref{single:sec:strong-ana}. %Discussion is given in Section \ref{single:sec:strong-diss}. 

==> s_urestls_app_lemmasubsec31.tex <==
First consider the case $(\hat{\psi}_t,u) \notin \textrm{Crit}(\boldsymbol{P})$. Then $\exists \epsilon_0>0$ such that $\textrm{MakeOpt}(\psi,u;\boldsymbol{P},\epsilon_0)=\emptyset$. On the event $F_t$ we have
\begin{align}
\left|\sum_{y \in S^u} V(\hat{\psi}_t,y,u) (\hat{h}_t ( T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,y,u))- h_{\boldsymbol{P}} ( T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,y,u))\right| \leq \epsilon, ~~ \forall u \in U, \tilde{P} \in \Xi. \label{s:urestls:eqn:reused1}
\end{align}
Thus for $\epsilon < \epsilon_0/3$,
\begin{align}
{\cal I}_t(\hat{\psi}_t,u) &\leq \sup_{\tilde{\boldsymbol{P}} \in \boldsymbol{\Xi}} \{\bar{r}(\hat{\psi}_t,u) + \sum_{y \in S^u} V(\hat{\psi}_t,y,u) \hat{h}_t (T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,y,u)) \} \notag \\
&\leq \sup_{\tilde{\boldsymbol{P}} \in \boldsymbol{\Xi}} \{\bar{r}(\hat{\psi}_t,u) + \sum_{y \in S^u} V(\hat{\psi}_t,y,u) h_{\boldsymbol{P}} (T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,y,u)) \} \notag \\
&< {\cal L}^*(\hat{\psi}_t,\boldsymbol{P}) - \epsilon_0 + \epsilon \notag \\
&< {\cal L}^*(\hat{\psi}_t,\boldsymbol{P}) -2\epsilon, \notag
\end{align}
%
which implies that
\begin{align*}
& I(\hat{\psi}_t \in J_l, U_t=u, E_t, F_t, {\cal I}(\hat{\psi}_t, u) \geq {\cal L}^*(\hat{\psi}_t,\boldsymbol{P}) - 2 \epsilon) = 0. 
\end{align*}

Next, we consider the case when $(\hat{\psi}_t,u) \in \textrm{Crit}(\boldsymbol{P})$. \revq{Note that by Lemma \ref{lemma:subsetoptimal}}, $\tau_{\textrm{tr}}$ can be selected such that the suboptimality gap for any belief in $J_l$, $l \in \{1,\ldots,A(\tau_{\textrm{tr}})\}$ is at least $\delta''>0$. Consider $(\psi,u) \in \textrm{Crit}(\boldsymbol{P}), \psi \in J_l$ for some $l \in \{1,\ldots,A(\tau_{\textrm{tr}})\}$. Let $3\epsilon = C \delta''$ where $0<C<1$ is some constant. We have
\begin{align*}
{\cal L}(\psi,u,h_{\boldsymbol{P}},\boldsymbol{P}) \leq {\cal L}^*(\psi,\boldsymbol{P}) - \delta''.
\end{align*}
Since $\textrm{MakeOpt}(\psi,u;\boldsymbol{P},C\delta'') \neq \emptyset$, for any $\tilde{\boldsymbol{P}}$ such that
\begin{align*}
{\cal L}(\psi,u,h_{\boldsymbol{P}},\tilde{\boldsymbol{P}}) \geq {\cal L}^*(\psi,\boldsymbol{P}) - C\delta'',
\end{align*}
we have
%
\begin{align*}
& {\cal L}(\psi,u,h_{\boldsymbol{P}},\tilde{\boldsymbol{P}}) - {\cal L}(\psi,u,h_{\boldsymbol{P}},\boldsymbol{P}) \geq (1-C)\delta'' \\
&\Rightarrow \sum_{y \in S^u} V(\psi,y,u) (h_{\boldsymbol{P}}(T_{\tilde{\boldsymbol{P}}}(\psi,y,u))-h_{\boldsymbol{P}}(T_{\boldsymbol{P}}(\psi,y,u))) \geq (1-C)\delta'' \\
&\Rightarrow \max_{y \in S^u} |(h_{\boldsymbol{P}}(T_{\tilde{\boldsymbol{P}}}(\psi,y,u))-h_{\boldsymbol{P}}(T_{\boldsymbol{P}}(\psi,y,u))| \geq (1-C)\delta'' \\
&\Rightarrow \left\|\tilde{\boldsymbol{P}}-\boldsymbol{P}\right\|_1 \geq 2\delta,
\end{align*}
%
for some $\delta>0$ by continuity of $h_{\boldsymbol{P}}$ and $T_{\boldsymbol{P}}$. Therefore $J_{\psi,u}(\boldsymbol{P};\boldsymbol{P},3\epsilon) > 2\delta$ for any $(\psi,u) \in \textrm{Crit}(\boldsymbol{P}), \psi \in J_l$ for some $l \in \{1,\ldots, A(\tau_{\textrm{tr}})\}$. Before proceeding, we also note that
%\begin{lemma} \label{lemma:contofj}
$J_{\psi,u}(\hat{\boldsymbol{P}};\boldsymbol{P},\epsilon)$ is continuous in its first argument. Therefore there exists a function $f_{\boldsymbol{P},\epsilon}$ such that $f_{\boldsymbol{P},\epsilon}(\delta)>0$ for $\delta>0$ and $\lim_{\delta \longrightarrow 0} f_{\boldsymbol{P},\epsilon}(\delta) =0$, for which $|J_{\psi,u}(\boldsymbol{P};\boldsymbol{P},\epsilon)-J_{\psi,u}(\hat{\boldsymbol{P}};\boldsymbol{P},\epsilon)|>\delta$ implies $\left\|\boldsymbol{P}-\hat{\boldsymbol{P}}\right\|_1 > f_{\boldsymbol{P},\epsilon}(\delta)$.
%\end{lemma}

The event $\{{\cal I}_t(\hat{\psi}_t,u) \geq {\cal L}^*(\hat{\psi}_t, \boldsymbol{P}) - 2\epsilon \}$ is equivalent to
%
\begin{align}
\exists \tilde{\boldsymbol{P}} \in \boldsymbol{\Xi}&: \left( \left\|\hat{\boldsymbol{P}}_t - \tilde{\boldsymbol{P}} \right\|_1^2 \leq \frac{2 \log t}{N_t(u)} \right), \notag \\
&(\bar{r}(\hat{\psi}_t, u) + ( V(\hat{\psi}_t,.,u) \bullet \hat{h}_t ( T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,.,u))) \geq {\cal L}^*(\hat{\psi}_t,\boldsymbol{P}) -2\epsilon ). \label{s:urestls:eqn:subsec311}
\end{align}
%
On the event $F_t$ we have
\begin{align*}
\left|\sum_{y \in S^u} V(\hat{\psi}_t,y,u) (\hat{h}_t ( T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,y,u))- h_{\boldsymbol{P}} ( T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,y,u))\right| \leq \epsilon, \forall u \in U, \tilde{\boldsymbol{P}} \in \boldsymbol{\Xi}. 
\end{align*}
Thus (\ref{s:urestls:eqn:subsec311}) implies
\begin{align}
\exists \tilde{\boldsymbol{P}} \in \boldsymbol{\Xi} &: \left( \left\|\hat{\boldsymbol{P}}_t - \tilde{\boldsymbol{P}} \right\|_1^2 \leq \frac{2 \log t}{N_t(u)}  \right), \notag \\
&( \bar{r}(\hat{\psi}_t, u)+ 
%\sum_{y \in S_u} V(\hat{\psi}_t,y,u) h^*_P ( T_{\tilde{P}}(\hat{\psi}_t,y,u)) \geq {\cal L}^*(\hat{\psi}_t,P) -3\epsilon \right) \label{eqn:subsec312}
( V(\hat{\psi}_t,.,u) \bullet h_{\boldsymbol{P}} ( T_{\tilde{\boldsymbol{P}}}(\hat{\psi}_t,.,u))) \geq {\cal L}^*(\hat{\psi}_t,\boldsymbol{P}) -3 \epsilon ). \label{s:urestls:eqn:subsec312}
\end{align}
From the definition of $J_{\psi,u}(\hat{\boldsymbol{P}};\boldsymbol{P},\epsilon)$ (\ref{s:urestls:eqn:subsec312}) implies
\begin{align}
J_{\hat{\psi}_t,u}(\hat{\boldsymbol{P}}_t;\boldsymbol{P},3\epsilon) \leq \frac{2 \log t}{N_t(u)}. \notag
\end{align}
Thus we have
\begin{align}
D_{1,1}(T,\epsilon,J_l,u) &\leq \sum_{t=0}^{T-1} I\left(\hat{\psi}_t \in J_l, U_t=u, J_{\hat{\psi}_t,u}(\hat{\boldsymbol{P}}_t;\boldsymbol{P},3\epsilon) \leq \frac{2 \log t}{N_t(u)}, (\hat{\psi}_t,u) \in \textrm{Crit}(\boldsymbol{P}),  E_t  \right) \notag \\
%&\leq& \sum_{t=0}^{N-1} I\left(\hat{\psi}_t \in J_l, U_t=u, J_{\hat{\psi}_t,u}(\hat{P}_t;P,3\epsilon) \leq \frac{2 \log t}{N_t(u)}, J_{\hat{\psi}_t,u}(P;P,3\epsilon) \leq J_{\hat{\psi}_t,u}(\hat{P}_t;P,3\epsilon)+\delta, E_t  \right) \notag \\
%&+& \sum_{t=0}^{N-1} I\left(\hat{\psi}_t \in J_l, U_t=u, J_{\hat{\psi}_t,u}(\hat{P}_t;P,3\epsilon) \leq \frac{2 \log t}{N_t(u)}, J_{\hat{\psi}_t,u}(P;P,3\epsilon) > J_{\hat{\psi}_t,u}(\hat{P}_t;P,3\epsilon)+\delta, E_t  \right) \notag \\
&\leq \sum_{t=0}^{T-1}  I\left(\hat{\psi}_t \in J_l, U_t=u ,E_t , (\hat{\psi}_t,u) \in \textrm{Crit}(\boldsymbol{P}) 
 J_{\hat{\psi}_t,u}(\boldsymbol{P};\boldsymbol{P},3\epsilon) \leq \frac{2 \log t}{N_t(u)} +\delta  \right) \label{s:urestls:eqn:subsec313} \\
&+ \sum_{t=0}^{T-1}  I\left(\hat{\psi}_t \in J_l, U_t=u, E_t, (\hat{\psi}_t,u) \in \textrm{Crit}(\boldsymbol{P})  
J_{\hat{\psi}_t,u}(\boldsymbol{P};\boldsymbol{P},3\epsilon) > J_{\hat{\psi}_t,u}(\hat{\boldsymbol{P}}_t;\boldsymbol{P},3\epsilon)+\delta \right). \label{s:urestls:eqn:subsec314}
\end{align}
Note that (\ref{s:urestls:eqn:subsec313}) is less than or equal to
\begin{align}
\frac{4 \log T}{\delta}. \label{s:urestls:eqn:subsec315}
\end{align}
%\begin{align}
%\sum_{t=0}^{N-1} I\left(\hat{\psi}_t \in J_l, U_t=u, , N_t(u) \leq \frac{2 \log t}{J_{\hat{\psi}_t,u}(P;P,3\epsilon)-\delta}, E_t  \right) \leq \frac{4 \log N}{\delta} \label{eqn:subsec315}
%\end{align}
By the continuity argument we mentioned above $J_{\hat{\psi}_t,u}(\boldsymbol{P};\boldsymbol{P},3\epsilon) > J_{\hat{\psi}_t,u}(\hat{\boldsymbol{P}}_t;\boldsymbol{P},3\epsilon)+\delta$ implies $\left\|\hat{\boldsymbol{P}}_t - \boldsymbol{P} \right\|_1 > f_{\boldsymbol{P},3\epsilon}(\delta)$. Thus (\ref{s:urestls:eqn:subsec314}) us upper bounded by
\begin{align*}
\sum_{t=0}^{T-1} I\left( \left\|\hat{\boldsymbol{P}}_t - \boldsymbol{P} \right\|_1 > f_{\boldsymbol{P},3\epsilon}(\delta), E_t \right).
\end{align*}
%
Taking expectation we have
%
\begin{align}
\sum_{t=0}^{T-1} P\left( \left\|\hat{\boldsymbol{P}}_t - \boldsymbol{P} \right\|_1 > f_{\boldsymbol{P},3\epsilon}(\delta), E_t \right)
&\leq \sum_{t=0}^{T-1} \sum_{k=1}^K \sum_{(i,j) \in S^k \times S^k} P\left(|\hat{p}^k_{ij,t} - p^k_{ij}| \geq \frac{f_{\boldsymbol{P},3\epsilon}(\delta)}{K S^2_{\max}}\right) \notag \\
\leq K S^2_{\max} \beta. \label{s:urestls:eqn:useful2}
\end{align}
%
Combining (\ref{s:urestls:eqn:subsec315}) and (\ref{s:urestls:eqn:useful2}) we have
%
\begin{align*}
E^{\boldsymbol{P}}_{\psi_0,\alpha}[D_{1,1}(T,\epsilon,J_l,u)] \leq (K S^2_{\max} +4/\delta) \beta.
\end{align*}



==> s_urestls_app_lemmasubsec33.tex <==
First we will relate $\left\|{\cal P}_{\boldsymbol{P},\gamma}-{\cal P}_{\hat{\boldsymbol{P}},\gamma} \right\|_1$ with $\left\|\boldsymbol{P}-\hat{\boldsymbol{P}}\right\|_1$. Let ${\cal P}_{\boldsymbol{P},\gamma}(i,j)$ be the $ij$th entry of ${\cal P}_{\boldsymbol{P},\gamma}$ which denotes the probability of transition from information state $i$ to $j$ under policy $\gamma$, and set of stochastic matrices $\boldsymbol{P}$. Note that from each $i$ it is possible to transition to only $\sum_{k \in {\cal K}} |S^k|$ different information states, and for each $j$ which is reachable from $i$ in one step there is a unique arm $l$ the agent should play at information state $i$ to get to $j$ with positive probability. Let $(s^{l},\tau^{l})$ denote the last observed state and time till last observation of arm $l$ in information state $i$ and $\bar{s}^{l}$ denote the state of arm $l$ in information state $j$. Then we have
%
\begin{align}
|{\cal P}_{\boldsymbol{P},\gamma}(i,j)-{\cal P}_{\hat{\boldsymbol{P}},\gamma}(i,j)| &= |((P^l)^{\tau^{l}} e^{l}_{s^l})_{\bar{s}^{l}} - ((\hat{P}^l)^{\tau_{l}} e^{l}_{s^l})_{\bar{s}^{l}}| \notag \\
&\leq \left\| (P^l)^{\tau^{l}} e^{l}_{s^l} - (\hat{P}^l)^{\tau^{l}} e^{l}_{s^l} \right\|_1 \notag \\
&\leq C_1(P^l, \infty) \left\|P^l - \hat{P}^l \right\|_1 ~. \notag
\end{align}
Since ${\cal P}_{\boldsymbol{P},\gamma}(i,j)$ and ${\cal P}_{\hat{\boldsymbol{P}},\gamma}(i,j)$ are nonzero for at most $\sum_{k \in K} |S^k|$ different information states, we have
%
\begin{align}
\left\|{\cal P}_{\boldsymbol{P},\gamma}-{\cal P}_{\hat{\boldsymbol{P}},\gamma} \right\|_1 \leq \sum_{k \in K} |S^k| \max_{k \in {\cal K}} \left(C_1(P^k, \infty) \left\|P^k - \hat{P}^k \right\|_1\right) ~. \label{s:urestls:eqn:hbound6}
\end{align}
The difference between the bias terms under $\boldsymbol{P}$ and $\hat{\boldsymbol{P}}$ can be written as
%
\begin{align}
|h_{\boldsymbol{P},\gamma}(i)-h_{\hat{\boldsymbol{P}},\gamma}(i)| &\leq \left|\sum_{t=1}^T \left[(e_i {\cal P}^{t-1}_{\boldsymbol{P},\gamma}) \tilde{r}^T_{\boldsymbol{P},\gamma} - (e_i {\cal P}^{t-1}_{\hat{\boldsymbol{P}},\gamma}) \tilde{r}^T_{\hat{\boldsymbol{P}},\gamma} \right]\right| \label{s:urestls:eqn:hbound1} \\
&+ T|g_{\boldsymbol{P},\gamma}-g_{\hat{\boldsymbol{P}},\gamma}| \label{s:urestls:eqn:hbound2} \\
&+ \left|\sum_{t=T+1}^\infty (e_i {\cal P}^{t-1}_{\boldsymbol{P},\gamma} - \pi^*_{\boldsymbol{P},\gamma})\tilde{r}^T_{\boldsymbol{P},\gamma} \right| + \left|\sum_{t=T+1}^\infty (e_i {\cal P}^{t-1}_{\hat{\boldsymbol{P}},\gamma} - \pi^*_{\hat{\boldsymbol{P}},\gamma})\tilde{r}^T_{\hat{\boldsymbol{P}},\gamma} \right|. \label{s:urestls:eqn:hbound3}
\end{align}
Consider (\ref{s:urestls:eqn:hbound1}). We have
%
\begin{align}
&\left|\sum_{t=1}^T \left[(e_i {\cal P}^{t-1}_{\boldsymbol{P},\gamma}) \tilde{r}^T_{\boldsymbol{P},\gamma} - (e_i {\cal P}^{t-1}_{\hat{\boldsymbol{P}},\gamma}) \tilde{r}^T_{\hat{\boldsymbol{P}},\gamma} \right]\right| \notag \\
&\leq \sum_{t=1}^T r_{\max} \left\|e_i {\cal P}^{t-1}_{\boldsymbol{P},\gamma} - e_i {\cal P}^{t-1}_{\hat{\boldsymbol{P}},\gamma} \right\|_1 \notag \\
&\leq \sum_{t=1}^T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma},t) \left\|{\cal P}_{\boldsymbol{P},\gamma}-{\cal P}_{\hat{\boldsymbol{P}},\gamma} \right\|_1 \label{s:urestls:eqn:hbound4} \\
&\leq T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma},\infty) \left\|{\cal P}_{\boldsymbol{P},\gamma}-{\cal P}_{\hat{\boldsymbol{P}},\gamma} \right\|_1, \label{s:urestls:eqn:hbound5} \\
&\leq T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma},\infty) \sum_{k \in {\cal K}} |S^k| \max_{k \in {\cal K}} \left(C_1(P^k, \infty) \left\|P^k - \hat{P}^k \right\|_1\right) \label{s:urestls:eqn:hbound7}
\end{align}
where (\ref{s:urestls:eqn:hbound4}) follows from Lemma \ref{intro:lemma:ergodic}, (\ref{s:urestls:eqn:hbound5}) follows from the fact that $C_1({\cal P}_{\boldsymbol{P},\gamma},t) \leq C_1({\cal P}_{\boldsymbol{P},\gamma},\infty)$ for all $t>0$, and (\ref{s:urestls:eqn:hbound7}) follows from (\ref{s:urestls:eqn:hbound6}). Thus given
%
\begin{align}
\left\|P^k - \hat{P}^k \right\|_1 \leq \frac{\epsilon}{3 T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma},\infty) \sum_{k \in {\cal K}} |S^k| \max_{k \in {\cal K}} \left(C_1(P^k, \infty)\right)}, \forall k \in {\cal K}, \notag
\end{align}
we have
\begin{align}
\left|\sum_{t=1}^T \left[(e_i {\cal P}^{t-1}_{\boldsymbol{P},\gamma}) \tilde{r}^T_{\boldsymbol{P},\gamma} - (e_i {\cal P}^{t-1}_{\hat{\boldsymbol{P}},\gamma}) \tilde{r}^T_{\hat{\boldsymbol{P}},\gamma} \right]\right|  \leq \frac{\epsilon}{3}. \label{s:urestls:eqn:hbound10}
\end{align}
Now consider (\ref{s:urestls:eqn:hbound2}). We have
%
\begin{align}
T |g_{\boldsymbol{P},\gamma}-g_{\hat{\boldsymbol{P}},\gamma}| &\leq T r_{\max} \left\| \pi^*_{\boldsymbol{P},\gamma} - \pi^*_{\hat{\boldsymbol{P}},\gamma}\right\|_1 \notag \\
&\leq  T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma}, \infty) \left\|{\cal P}_{\boldsymbol{P},\gamma}-{\cal P}_{\hat{\boldsymbol{P}},\gamma}\right\|_1 \label{s:urestls:eqn:hbound8} \\
&\leq T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma}, \infty) \sum_{k \in {\cal K}} |S^k| \max_{k \in {\cal K}} \left(C_1(P^k, \infty) \left\|P^k - \hat{P}^k \right\|_1\right), \label{s:urestls:eqn:hbound9}
\end{align}
where (\ref{s:urestls:eqn:hbound8}) follows from Lemma \ref{intro:lemma:ergodic}, and (\ref{s:urestls:eqn:hbound9}) follows from (\ref{s:urestls:eqn:hbound6}). Thus given
%
\begin{align}
\left\|P^k - \hat{P}^k \right\|_1 \leq \frac{\epsilon}{3 T r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma},\infty) \sum_{k \in {\cal K}} |S^k| \max_{k \in {\cal K}} \left(C_1(P^k, \infty)\right)}, \forall k \in {\cal K}, \notag
\end{align}
we have
\begin{align}
T |g_{\boldsymbol{P},\gamma}-g_{\hat{\boldsymbol{P}},\gamma}| \leq \frac{\epsilon}{3}. \label{s:urestls:eqn:hbound11}
\end{align}

Finally, consider (\ref{s:urestls:eqn:hbound3}). Using uniform ergodicity, $\exists C<\infty, \rho<1$ such that $\left\|e_i {\cal P}^t_{\boldsymbol{P},\gamma} - \pi^*_{\boldsymbol{P},\gamma}\right\|_1 \leq C \rho^t$ and $\left\|e_i {\cal P}^t_{\hat{\boldsymbol{P}},\gamma} - \pi^*_{\hat{\boldsymbol{P}},\gamma}\right\|_1 \leq C \rho^t$. Then
\begin{align}
& \left|\sum_{t=T+1}^\infty (e_i {\cal P}^{t-1}_{\boldsymbol{P},\gamma} - \pi^*_{\boldsymbol{P},\gamma}) \tilde{r}^T_{\boldsymbol{P},\gamma} \right| + \left|\sum_{t=T+1}^\infty (e_i {\cal P}^{t-1}_{\hat{\boldsymbol{P}},\gamma} - \pi^*_{\hat{\boldsymbol{P}},\gamma}) \tilde{r}^T_{\hat{\boldsymbol{P}},\gamma} \right| \notag \\
&\leq \sum_{t=T+1}^\infty r_{\max} \left\|e_i {\cal P}^t_{\boldsymbol{P},\gamma} - \pi^*_{\boldsymbol{P},\gamma}\right\|_1 + \sum_{t=T+1}^\infty r_{\max} \left\|e_i {\cal P}^t_{\hat{\boldsymbol{P}},\gamma} - \pi^*_{\hat{\boldsymbol{P}},\gamma}\right\|_1 \notag \\
&\leq 2 r_{\max} C \frac{\rho^T}{1-\rho} ~. \notag
\end{align}
Let $T_0>0$ be such that
\begin{align}
2 r_{\max} C \frac{\rho^{T_0}}{1-\rho} \leq \frac{\epsilon}{3} ~. \label{s:urestls:eqn:hbound12}
\end{align}
Then for
%
\begin{align}
\left\|P^k - \hat{P}^k \right\|_1 \leq \frac{\epsilon}{3 T_0 r_{\max} C_1({\cal P}_{\boldsymbol{P},\gamma},\infty) \sum_{k \in {\cal K}} |S^k| \max_{k \in {\cal K}} \left(C_1(P^k, \infty)\right)}, \forall k \in {\cal K} ~, \notag
\end{align}
using the results in (\ref{s:urestls:eqn:hbound10}), (\ref{s:urestls:eqn:hbound11}) and (\ref{s:urestls:eqn:hbound12}), we have
%
\begin{align}
|h_{\boldsymbol{P},\gamma}(i)-h_{\hat{\boldsymbol{P}},\gamma}(i)| \leq \epsilon, ~\forall i \in \Psi_C ~, \notag
\end{align}
which implies
%
\begin{align}
\left\|h_{\boldsymbol{P},\gamma}-h_{\hat{\boldsymbol{P}},\gamma} \right\|_\infty \leq \epsilon ~. \notag
\end{align}
% 

==> strong_extension.tex <==
In this section we propose several extensions to ALA and relaxation of certain assumptions. Firstly, we consider an adaptive exploration function for ALA, by which the player can achieve near-logarithmic regret without knowing a sufficient bound on the distance between the true and estimated transition probabilities (such that the exploration constant $L$ can be chosen large enough). Secondly, we present a modified algorithm for which Assumption \ref{s:urestls:assump:esuboptimality} can be relaxed. We prove that the modified algorithm can achieve logarithmic regret without Assumption \ref{s:urestls:assump:esuboptimality}.

\subsection{An adaptive exploration function}

We note that the analysis in Section \ref{single:sec:strong-analysis} holds when ALA is run with a sufficiently large exploration constant $L$ such that at each exploitation step the estimated transition probabilities $\hat{\boldsymbol{P}}$ is close enough to $\boldsymbol{P}$ to guarantee that all regret terms in (\ref{s:urestls:eqn:regretbound}) is finite except the regret due to explorations which is logarithmic in time. In other words, there is an $L_0(\boldsymbol{P}) > 0$ such that when ALA is run with $L \geq L_0(\boldsymbol{P})$ , at the end of each exploration step we have $||\hat{\boldsymbol{P}} - \boldsymbol{P}||_1 \leq \delta(\boldsymbol{P})$, where $\delta(\boldsymbol{P})>0$ is a constant for which Theorem \ref{s:urestls:theorem:main} holds.  

However, in our learning model we assumed that the player does not know the transition probabilities initially, therefore it is impossible for the player to check if $L \geq L_0(\boldsymbol{P})$. Let $\tilde{\boldsymbol{\Xi}} \subset \boldsymbol{\Xi}$ be the set of transition probability matrices where $\boldsymbol{P}$ lies in. If the player knows $\tilde{\boldsymbol{\Xi}}$, then it can compute $\tilde{L}_0 = \sup_{\tilde{\boldsymbol{P}} \in \tilde{\boldsymbol{\Xi}}} L_0(\tilde{\boldsymbol{P}})$, and choose $L > \tilde{L}_0$. 

In this section, we present another exploration function for ALA such that the player can achieve near-logarithmic regret even without knowing $L_0(\boldsymbol{P})$ or $\tilde{L}_0$. Let $f(t) = L(t) \log t$ where $L(t)$ is an increasing function such that $L(1)=1$ and $\lim_{t \rightarrow \infty} L(t) = \infty$. The intuition behind this exploration function is that after some time $T_0$, $L(t)$ will be large enough so that the estimated transition probabilities are sufficiently accurate, and the regret due to incorrect calculations is a constant independent of time. 

\begin{theorem}
%
When $\boldsymbol{P}$ is such that Assumptions \ref{s:urestls:assump:1} and \ref{s:urestls:assump:esuboptimality2} hold. If the player uses ALA with $f(t) = L(t) \log t$, for some $L(t)$ such that $L(1)=1$ and $\lim_{t \rightarrow \infty} L(t) = \infty$, then there exists constant $\delta(L) > 0$, $\tau^0(\boldsymbol{P}) > 0$, $T_0(L, \boldsymbol{P})>0$ such that the regret is upper bounded by
%
\begin{align*}
R^{\alpha}_{\psi_0; \boldsymbol{P}}(T) & \leq r_{\max} \left( T_0(L, \boldsymbol{P}) + \left(\sum_{k=1}^K |S^k| \right) L(T) \log T (1+T_{\max}) \right. \\
&\left. +(8 K S^2_{\max} + 4/\delta(L)) \beta 
\left( \sum_{l=1}^{A(\tau^0)} \sum_{u \notin O(J_l;\boldsymbol{P})}  \bar{\Delta}(J_l, u; \boldsymbol{P})\right) \right)  \\ 
&\leq r_{\max} \left( T_0(L, \boldsymbol{P}) + \left(\sum_{k=1}^K |S^k| \right) L(T) \log T (1+T_{\max}) \right. \\
& \left. + (8 K S^2_{\max} + 4/\delta(L))\beta 
 (\tau^0)^M  \left(\sum_{k=1}^K |S^k| \right) \max_{l \in \{1,\ldots, A(\tau^0) \}}  \bar{\Delta}(J_l, u; \boldsymbol{P})
 \right) 
\end{align*}
%
\end{theorem}
%
\begin{proof}
The regret up to $T_0(L, \boldsymbol{P})$ can be at most $r_{\max} T_0(L, \boldsymbol{P})$. After $T_0(L, \boldsymbol{P})$, since $L(t) \geq L_0(\boldsymbol{P})$, transition probabilities at exploitation steps sufficiently accurate so that all regret terms in (\ref{s:urestls:eqn:regretbound}) except the regret due to explorations is finite. Since time $t$ is an exploration step whenever $C^k_i(t) < L(t) \log t$, the regret due to explorations is
%
\begin{align*}
r_{\max} \left(\sum_{k=1}^K |S^k| \right) L(T) \log T (1+T_{\max})
\end{align*}
%
\end{proof}

\begin{remark}\label{remark:unknowngap}
There is a tradeoff between choosing a rapidly increasing $L$ or a slowly increasing $L$. The regret of ALA up to time $T_0(L, \boldsymbol{P})$ is linear. Since $T_0(L, \boldsymbol{P})$ is decreasing in function $L$, a rapidly increasing $L$ will have better performance when the considered time horizon is small. However, in terms of asymptotic performance, i.e., as $T \rightarrow 
\infty$, $L$ should be a slowly diverging sequence. For example if $L = \log(\log t)$, then the asymptotic regret will be $O(\log(\log t) \log t )$. 
\end{remark}
 
 
\subsection{Adaptive Learning Algorithm with Finite Partitions}

In this section, we consider a variant of ALA which is called adaptive learning algorithm with finite partitions (ALA-FP). We show that ALA-FP achieves logarithmic regret even when Assumption \ref{s:urestls:assump:esuboptimality} does not hold. Basically, ALA-FP takes as input the mixing time $\tau^0$, then forms ${\cal G}_{\tau^0}$ partition of the set of information states ${\cal C}$. At each exploitation step ALA-FP solves the estimated AROE based on the transition probability estimated $\hat{\boldsymbol{P}}$, and if the belief $(\boldsymbol{s}, \boldsymbol{\tau})$ is in  $G_l$, the player arbitrarily picks an arm in $O^*(G_l; \hat{\boldsymbol{P}})$, instead of picking an arm in $O(\psi_{\hat{\boldsymbol{P}}}((\boldsymbol{s}, \boldsymbol{\tau})); \hat{\boldsymbol{P}})$. When time $t$ is an exploitation step, the player  plays optimally by choosing an arm in $O(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau})); \boldsymbol{P})$, or near-optimally by choosing an arm in $O^*(G_l; \boldsymbol{P})$ different from $O(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau})); \boldsymbol{P})$ such that $(\boldsymbol{s}, \boldsymbol{\tau}) \in G_l$, or suboptimally by choosing an arm that is neither in $O(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau})); \boldsymbol{P})$ nor in $O^*(G_l; \boldsymbol{P})$. By Lemma \ref{lemma:subsetoptimal} we know that when $\tau^0$ is chosen large enough, for any $G_l \in {\cal G}_{\tau^0}$, and $(\boldsymbol{s}, \boldsymbol{\tau})$, $O(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau})); \boldsymbol{P})$ is a subset of $O^*(G_l; \boldsymbol{P})$. Since the solution to the AROE is a continuous function, by choosing a large enough $\tau^0$, we can control the regret due to near-optimal actions. The regret due to suboptimal actions can be bounded the same way as in Theorem \ref{s:urestls:theorem:main}. The following theorem gives a logarithmic upper bound on the regret of ALA-FP. 

\begin{theorem} \label{thm:finite_partition}
When the true set of transition probabilities $\boldsymbol{P}$ is such that Assumption \ref{s:urestls:assump:1} is true, for a player using ALA-FP with exploration constant $L$, and mixing time $\tau^0$ sufficiently large such that for any $(\boldsymbol{s}, \boldsymbol{\tau}) \in G_l$, $G_l \in {\cal G}_{\tau^0}$, we have $|h_{\boldsymbol{P}}(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau}))) - h_{\boldsymbol{P}}(\psi^*(G_l; \boldsymbol{P}))|< C/2T$, where $C$ is a constant and $T$ is the time horizon, the regret of ALA-FP is upper bounded by
%
\begin{eqnarray}
R^{\alpha}_{\psi_0; \boldsymbol{P}}(T) &\leq C + (L \log T (1+T_{\max}) +(8 K S^2_{\max} + 4/\delta)\beta)
\times \sum_{l=1}^{A(\tau^0)} \sum_{u \notin O(J_l;\boldsymbol{P})}  \bar{\Delta}(J_l, u; \boldsymbol{P}), \nonumber
\end{eqnarray}
for some $\delta > 0$ which depends on $L$ and $\tau^0$.
\end{theorem}
%
\begin{proof} %PROOF OF theorem:main
The regret at time $T$ is upper bounded by (\ref{eqn:defnregret}). Consider any $t$ which is an exploitation step. Let $l$ be such that $(\boldsymbol{s}_t, \boldsymbol{\tau}_t) \in G_l$. If the selected arm $\alpha(t) \in O(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau})); \boldsymbol{P})$, then an optimal decision is made at $t$, so the contribution to regret in time step $t$ is zero. Next, we consider the case when $\alpha(t) \notin O(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau})); \boldsymbol{P})$. In this case there are two possibilities. Either $\alpha(t) \in O^*(G_l; \boldsymbol{P})$ or not. We know that when $O^*(G_l; \hat{\boldsymbol{P}}_t) \subset O^*(G_l; \boldsymbol{P})$ we have $\alpha(t) \in O^*(G_l; \boldsymbol{P})$. Since $|h_{\boldsymbol{P}}(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau}))) - h_{\boldsymbol{P}}(\psi^*(G_l; \boldsymbol{P}))|< C/2T$ for all $(\boldsymbol{s}, \boldsymbol{\tau}) \in G_l$, we have by (\ref{s:urestls:eqn:suboptimality}),
%
\begin{align}
\Delta(\psi_t ,\alpha(t) ;\boldsymbol{P}) &= {\cal L}^*(\psi_t,\boldsymbol{P}) - {\cal L}(\psi_t,\alpha(t),h_{\boldsymbol{P}},\boldsymbol{P}) \leq C/T.
\end{align}
% 
Therefore, contribution of a near-optimal action to regret is at most $C/T$. 

Finally, consider the case when $\alpha(t) \notin O^*(G_l; \boldsymbol{P})$. This implies that either the estimated belief $\hat{\psi}_t$ is not close enough to $\psi_t$ or the estimated solution to the AROE $\hat{h}_t$ is not close enough to $h_{\boldsymbol{P}}$. Due to the non-vanishing suboptimality gap at any belief vector $\psi^*(G_l; \boldsymbol{P})$, and since decisions of ALA-FP is only based on belief vectors corresponding to $(\boldsymbol{s}, \boldsymbol{\tau}) \in {\cal C}$, the regret due to suboptimal actions can be bounded by Theorem \ref{s:urestls:theorem:main}. We get the regret bound by combining all these results.
\end{proof} 

Note that the regret bound in Theorem \ref{thm:finite_partition} depends on $\tau^0$ which depends on $T$ since $\tau^0$ should be chosen large enough so that for every $G_l$ in the partition created by $\tau^0$, function $h_{\boldsymbol{P}}$ should vary by at most $C/2T$. Clearly since $h_{\boldsymbol{P}}$ is a continuous function, the variation of $h_{\boldsymbol{P}}$ on $G_l$ decreases with the diameter of $G_l$ on the belief space. Note that there is a term in regret that depends linearly on the number of sets $A(\tau^0)$ in the partition generated by $\tau^0$, and $A(\tau^0)$ increases proportional to $(\tau^0)^M$. This tradeoff is not taken into account in Theorem \ref{thm:finite_partition}. For example, if $(\tau^0)^M \geq T$ then the regret bound in Theorem \ref{thm:finite_partition} is useless. Another approach is to jointly optimize the regret due to suboptimal and near-optimal actions by balancing the number of sets $A(\tau^0)$ and the variation of $h_{\boldsymbol{P}}$ on sets in partition ${\cal G}_{\tau^0}$. For example given $0<\theta \leq 1$, we can find a $\tau^0(\theta)$ such that for any $(\boldsymbol{s}, \boldsymbol{\tau}) \in G_l$, $G_l \in {\cal G}_{\tau^0(\theta)}$ we have $|h_{\boldsymbol{P}}(\psi_{\boldsymbol{P}}((\boldsymbol{s}, \boldsymbol{\tau}))) - h_{\boldsymbol{P}}(\psi^*(G_l; \boldsymbol{P}))|< C/(2T^{\theta})$. Then, the regret due to near-optimal decisions will be proportional to $C T^{1-\theta}$, and the regret due to suboptimal decision will be proportional to $(\tau^0(\theta))^M$. Let $C = \sup_{\psi \in \boldsymbol{\Psi}} h_{\boldsymbol{P}}(\psi) - \inf_{\psi \in \boldsymbol{\Psi}} h_{\boldsymbol{P}}(\psi)$. Since $T^{1-\theta}$ is decreasing in $\theta$ and $\tau^0(\theta)$ is increasing in $\theta$, there exists $\theta \in [0,1]$, such that $\theta = \arg\min_{\theta' \in [0,1]} |T^{1-\theta} - (\tau^0(\theta))^M|$ and $|T^{1-\theta} - (\tau^0(\theta))^M| \leq (\tau^0(\theta)+1)^M - (\tau^0(\theta))^M$. If the optimal value of $\theta$ is in $(0,1)$, then given $\theta$, the player can balance the tradeoff, and achieve sublinear regret proportional to $T^{1-\theta}$. However, since the player does not know $\boldsymbol{P}$ initially, it may not know the optimal value of $\theta$. Online learning algorithms for the player to estimate the optimal value of $\theta$ is a future research direction.



